A Large-Scale Exploratory Study of Android Sports Apps in the Google Play Store

Prior studies on mobile app analysis often analyze apps across different categories or focus on a small set of apps within a category. These studies either provide general insights for an entire app store which consists of millions of apps, or provide specific insights for a small set of apps. However, a single app category can often contain tens of thousands to hundreds of thousands of apps. For example, according to AppBrain, there are 46,625 apps in the "Sports" category of Google Play apps. Analyzing such a targeted category of apps can provide more specific insights than analyzing apps across categories while still benefiting many app developers interested in the category. This work aims to study a large number of apps from a single category (i.e., the sports category). We performed an empirical study on over two thousand sports apps in the Google Play Store. We study the characteristics of these apps (e.g., their targeted sports types and main functionalities) through manual analysis, the topics in the user review through topic modeling, as well as the aspects that contribute to the negative opinions of users through analysis of user ratings and sentiment. It is concluded that analyzing a targeted category of apps (e.g., sports apps) can provide more specific insights than analyzing apps across different categories while still being relevant for a large number (e.g., tens of thousands) of apps. Besides, as a rapid-growing and competitive market, sports apps provide rich opportunities for future research, for example, to study the integration of data science or machine learning techniques in software applications or to study the factors that influence the competitiveness of the apps.

==> texfiles/abstract.tex <==
\begin{abstract}
Prior studies on mobile app analysis often analyze apps across different categories or focus on a small set of apps within a category. These studies either provide general insights for an entire app store which consists of millions of apps or provide specific insights for a small set of apps.
However, a single app category can often contain tens of thousands to hundreds of thousands of apps. For example, according to AppBrain, there are 46,625 apps in the ``Sports'' category of Google Play apps.
Analyzing such a targeted category of apps can provide more specific insights than analyzing apps cross categories, while still benefit a very large number of app developers interested in the category.
In this work, we perform an empirical study on over two thousand sports apps in the Google Play Store. We analyze the characteristics of these apps (e.g., their main functionalities), the user reviews, as well as the aspects that contribute to the negative opinions of users.
Our work provides three folds of contributions: 1) we identified insights that are specifics for tens of thousands of sports apps; 2) we provide empirical evidence on the benefits of analyzing apps in a specific category; and 3) provide lessons learned from sports apps development that can benefit general app development.
\end{abstract}

==> texfiles/images/allsentiment-topic-updated-aug12.tex <==
\begin{table}[]
\caption{Sentiment and negative review distribution on different topics of entire dataset 
% \heng{put the table in results} \heng{it looks strange that Advertisement has one of the best sentiment, and positive feedback has a high percentage of negative reviews, please double check the result}}\bhagya{I have looked into the results, there are reviews with neutral and positive feedback with a mention of the issues with the advertisement}\bhagya{similarly the issue with the positive feedback is the category of the apps with highest number of reviews- thus the the number of negative sentiment is also higher ( issues with imbalanced class)} \heng{The number of the reviews does not matter, as you are measuring the percentage, right? Comparing this table 4 and table 3 in RQ2, it seems the percentage of negative reviews here is highly correlated with the topic percentage in Table 3. Are you calculating the percentage here this way: for example, for the ``positive fedback'' topic, divide the number of negative reviews with the ``positive feedback'' by the number of reviews with the ``positive feedback'' topic? It seems something is wrong here. }
\bhagya{updated}
}
\label{tab:allsentireview}
\centering
\scalebox{0.8}{
\begin{tabular}{@{}|l|c|c|@{}}
\toprule
\textit{\textbf{Topics}} & \multicolumn{1}{l|}{\textbf{Average sentiment}} & \multicolumn{1}{l|}{\textbf{percentage negative review}} \\ \midrule
Return on Investment & 0.5 & 0.35\% \\ \midrule
Positive Feedback & 0.44 & 0.58\% \\ \midrule
Quality of Content & 0.33 & 0.52\% \\ \midrule
Feature Request & 0.26 & 0.63\% \\ \midrule
Impact of Application & 0.21 & 1.18\% \\ \midrule
Review credibility & 0.17 & 0.69\% \\ \midrule
Negative Feedback & 0.15 & 0.73\% \\ \midrule
Video streaming quality & 0.1 & 1.77\% \\ \midrule
Accuracy of prediction & 0.08 & 1.44\% \\ \midrule
Advertisement & 0.08 & 0.92\% \\ \midrule
bug report & 0.08 & 1.02\% \\ \midrule
upto-date-ness & 0.06 & 2.98\% \\ \midrule
Version update & 0.03 & 2.31\% \\ \midrule
Precision of Tools & -0.02 & 1.23\% \\ \bottomrule
\end{tabular}}

\end{table}




==> texfiles/images/category-label-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{adjustbox}
\begin{table}[!t]
\centering
\caption{Characteristics of the manual analyzed sports apps: type of sports, main functionality, analytics approach.}
\begin{tabular}{@{}|p{2.6cm}|p{3cm}|c|@{}}
\toprule
\textbf{Classification category}                         & \textbf{Labels}   & \textbf{Distribution}                    \\ \midrule
                                                         & \textbf{Football} & \textbf{36.16\%} \\ \cmidrule(l){2-3} 
                                    & \textbf{General}                              & \textbf{23.73\%} \\ \cmidrule(l){2-3} 
                                    & Fitness                                       & 15.25\%          \\ \cmidrule(l){2-3} 
                                    & Golf                                          & 9.04\%           \\ \cmidrule(l){2-3} 
                                    & Basketball                                    & 5.08\%           \\ \cmidrule(l){2-3} 
                                    & Car Racing                                    & 1.69\%           \\ \cmidrule(l){2-3} 
                                    & Martial Arts                                  & 1.69\%           \\ \cmidrule(l){2-3} 
                                    & American Football                             & 1.13\%           \\ \cmidrule(l){2-3} 
                                    & Baseball                                      & 1.13\%           \\ \cmidrule(l){2-3} 
                                    & Cricket                                       & 1.13\%           \\ \cmidrule(l){2-3} 
                                    & NA                                            & 1.13\%           \\ \cmidrule(l){2-3} 
                                    & Athletics                                     & 0.56\%           \\ \cmidrule(l){2-3} 
                                    & Football and Basketball                       & 0.56\%           \\ \cmidrule(l){2-3} 
                                    & Game                                          & 0.56\%           \\ \cmidrule(l){2-3} 
                                    & Hockey                                        & 0.56\%           \\ \cmidrule(l){2-3} 
\multirow{-16}{*}{Domain of sports} & Wrestling                                     & 0.56\%           \\ \midrule
                                    & \textbf{Betting Tips}                         & \textbf{24.86\%} \\ \cmidrule(l){2-3} 
                                    & \textbf{Training}                             & \textbf{24.86\%} \\ \cmidrule(l){2-3} 
                                    & Live updates                                  & 15.25\%          \\ \cmidrule(l){2-3} 
                                    & Streaming                                     & 10.73\%          \\ \cmidrule(l){2-3} 
                                    & Tools                                         & 7.34\%           \\ \cmidrule(l){2-3} 
                                    & Tracking                                      & 4.52\%           \\ \cmidrule(l){2-3} 
                                    & Betting                                       & 3.39\%           \\ \cmidrule(l){2-3} 
                                    & News                                          & 2.82\%           \\ \cmidrule(l){2-3} 
                                    & Social Network                                & 2.26\%           \\ \cmidrule(l){2-3} 
                                    & League Management                             & 1.13\%           \\ \cmidrule(l){2-3} 
                                    & Radio                                         & 1.13\%           \\ \cmidrule(l){2-3} 
                                    & Team management                               & 1.13\%           \\ \cmidrule(l){2-3} 
\multirow{-13}{*}{Main functionality}    & Health Tips                                   & 0.56\%           \\ \midrule
                                    & Predictive analysis                           & 18.08\%          \\ \cmidrule(l){2-3} 
                                    & Analytical statistics                         & 7.34\%           \\ \cmidrule(l){2-3} 
                                    & Descriptive statistics                        & 7.34\%           \\ \cmidrule(l){2-3} 
                                    & \specialcell{Analytical statistics \\and Predictive analysis} & 3.95\%           \\ \cmidrule(l){2-3} 
                                    & Unknown                                       & 1.13\%           \\ \cmidrule(l){2-3} 

\multirow{-6}{*}{Used analytical method} & \textbf{NA}       & \textbf{62.15\%}                         \\ \bottomrule
\end{tabular}
\end{table}
\end{adjustbox}

==> texfiles/images/senti-func-topi-final.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

%\begin{table*}[!t]
\begin{sidewaystable}
%\begin{adjustbox}{angle=90} 
\centering
\small

\caption{Distribution of average review sentiment over different topics and different functionalities of sports apps. Also the percentage of negative sentiment reviews out of all reviews.} %\heng{all sentiment values are positive. the results are not quite helpful for answering the RQ: what are people complaining about? In addition to the average sentiment values, add the percentage of reviews with negative sentiment (what's the threshold used for tagging a negative sentiment, 0.05?). For example, put 10.23\% (0.20) where 10.23\% indicates the percentage of reviews of a app category and a topic that have negative sentiment, 0.20 indicate the average sentiment of all reviews of the app category and the topic.}
\label{tab:topic-function-senti}
\heng{for each app category, highlight the top three topics with highest percentage of reviews with negative sentiment}
%\heng{how to explain the positive feedback topic has the highest percentage of negative reviews? double check the result}
%\heng{here the grand total are for the sampled apps right? need a separate table for the topic sentiment of all 2,058 apps, similar to this table but only showing overall topic - sentiment (average sentiment and percentage of negative reviews). Then the grand total row can be removed from here (duplicated information).}\bhagya{I don't think it will be a duplicate information rather it shows the difference in distribution with the sample set and the whole dataset}\bhagya{updated rest of the comments}
\heng{similar comments as for Table 4: check the results }
\scalebox{0.48}{
\begin{tabular}{@{}|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|l|@{}}
\toprule
\textit{\textbf{Function}} & \multicolumn{1}{l|}{\textbf{\specialcell{Accuracy\\of Models}}} & \multicolumn{1}{l|}{\textbf{{\specialcell{Advertisement}}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Bug\\reports}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Feature\\Request}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Impact\\of Application}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Negative\\Feedback}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Positive\\Feedback}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Precision\\of\\Tools}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Quality\\of\\Content}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Return\\on\\Investment}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Review\\credibility}}} & \multicolumn{1}{l|}{\textbf{\specialcell{up-to-\\dateness}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Version\\update}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Video\\streaming\\quality}}}& \textbf{\specialcell{Grand\\Total}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Betting}} & \multicolumn{1}{c|}{0.55(0.311\%)} & \multicolumn{1}{c|}{0.61(0\%)} & \multicolumn{1}{c|}{0(0.13\%)} & \multicolumn{1}{c|}{\textbf{0.54(0.519\%)}} & \multicolumn{1}{c|}{0.53(0.052\%)} & \multicolumn{1}{c|}{0.2(0.078\%)} & \multicolumn{1}{c|}{\textbf{0.27(3.736\%)}} & \multicolumn{1}{c|}{0.42(0.052\%)} & \multicolumn{1}{c|}{\textbf{0.31(0.778\%)}} & \multicolumn{1}{c|}{0.44(0\%)} & \multicolumn{1}{c|}{0.48(0.104\%)} & \multicolumn{1}{c|}{0.13(0.441\%)} & \multicolumn{1}{c|}{0.45(0\%)} & \multicolumn{1}{c|}{0.24(0.441\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.37\\(0.474\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Betting\\Tips}}} & \multicolumn{1}{c|}{0.52(0.241\%)} & \multicolumn{1}{c|}{0.59(0.008\%)} & \multicolumn{1}{c|}{\textbf{0.15(1.932\%)}} & \multicolumn{1}{c|}{0.57(0.084\%)} & \multicolumn{1}{c|}{0.56(0\%)} & \multicolumn{1}{c|}{0.15(0.414\%)} & \multicolumn{1}{c|}{\textbf{0.34(3.112\%)}} & \multicolumn{1}{c|}{0.39(0.015\%)} & \multicolumn{1}{c|}{0.35(0.414\%)} & \multicolumn{1}{c|}{0.16(0.008\%)} & \multicolumn{1}{c|}{0.47(0.031\%)} & \multicolumn{1}{c|}{\textbf{0.21(2.637\%)}} & \multicolumn{1}{c|}{0.44(0.054\%)} & \multicolumn{1}{c|}{0.28(0.245\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.37\\(0.657\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Health\\Tips}}} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{c|}{0.75(0\%)} & \multicolumn{1}{c|}{0.14(0.08\%)} & \multicolumn{1}{c|}{0.49(0.08\%)} & \multicolumn{1}{c|}{0.56(0\%)} & \multicolumn{1}{c|}{\textbf{0.09(0.962\%)}} & \multicolumn{1}{c|}{\textbf{0.47(1.885\%)}} & \multicolumn{1}{c|}{0.32(0\%)} & \multicolumn{1}{c|}{0.42(0.16\%)} & \multicolumn{1}{c|}{0.06(0\%)} & \multicolumn{1}{c|}{0.56(0\%)} & \multicolumn{1}{c|}{\textbf{0.39(1.323\%)}} & \multicolumn{1}{c|}{0.45(0.241\%)} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.41\\(0.338\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{League\\Management}}} & \multicolumn{1}{c|}{0.49(0.386\%)} & \multicolumn{1}{c|}{0.78(0\%)} & \multicolumn{1}{c|}{0.48(0.386\%)} & \multicolumn{1}{c|}{\textbf{0.5(0.772\%)}} & \multicolumn{1}{c|}{0.53(0\%)} & \multicolumn{1}{c|}{0.01(0.386\%)} & \multicolumn{1}{c|}{\textbf{0.49(1.158\%)}} & \multicolumn{1}{c|}{0.38(0\%)} & \multicolumn{1}{c|}{0.4(0\%)} & \multicolumn{1}{c|}{0.03(0\%)} & \multicolumn{1}{c|}{0.62(0\%)} & \multicolumn{1}{c|}{0.27(0\%)} & \multicolumn{1}{c|}{0.41(0\%)} & \multicolumn{1}{c|}{0.43(0\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.42\\(0.221\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Live\\updates}}} & \multicolumn{1}{c|}{0.61(0.065\%)} & \multicolumn{1}{c|}{0.6(0.007\%)} & \multicolumn{1}{c|}{0.2(0.08\%)} & \multicolumn{1}{c|}{0.58(0.065\%)} & \multicolumn{1}{c|}{0.49(0.065\%)} & \multicolumn{1}{c|}{0.11(0.567\%)} & \multicolumn{1}{c|}{\textbf{0.57(0.771\%)}} & \multicolumn{1}{c|}{0.42(0\%)} & \multicolumn{1}{c|}{\textbf{0.32(0.625\%)}} & \multicolumn{1}{c|}{0.26(0.138\%)} & \multicolumn{1}{c|}{0.44(0.058\%)} & \multicolumn{1}{c|}{\textbf{0.42(0.778\%)}} & \multicolumn{1}{c|}{0.45(0.029\%)} & \multicolumn{1}{c|}{0.31(0.262\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.41\\(0.251\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{News}} & \multicolumn{1}{c|}{0.58(0.159\%)} & \multicolumn{1}{c|}{0.49(0.023\%)} & \multicolumn{1}{c|}{0.33(0.061\%)} & \multicolumn{1}{c|}{0.58(0.045\%)} & \multicolumn{1}{c|}{0.44(0.03\%)} & \multicolumn{1}{c|}{0.39(0.144\%)} & \multicolumn{1}{c|}{\textbf{0.54(0.605\%)}} & \multicolumn{1}{c|}{0.44(0.038\%)} & \multicolumn{1}{c|}{\textbf{0.25(1.286\%)}} & \multicolumn{1}{c|}{\textbf{0.37(2.292\%)}} & \multicolumn{1}{c|}{0.44(0.045\%)} & \multicolumn{1}{c|}{0.37(0.34\%)} & \multicolumn{1}{c|}{0.43(0.068\%)} & \multicolumn{1}{c|}{0.43(0.182\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.43\\(0.38\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Radio}} & \multicolumn{1}{c|}{0.5(0.225\%)} & \multicolumn{1}{c|}{0.64(0\%)} & \multicolumn{1}{c|}{0.01(0.045\%)} & \multicolumn{1}{c|}{0.53(0.045\%)} & \multicolumn{1}{c|}{\textbf{0.37(0.54\%)}} & \multicolumn{1}{c|}{0.31(0.135\%)} & \multicolumn{1}{c|}{\textbf{0.46(0.9\%)}} & \multicolumn{1}{c|}{0.45(0.135\%)} & \multicolumn{1}{c|}{\textbf{0.26(1.125\%)}} & \multicolumn{1}{c|}{0.58(0\%)} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{c|}{0.33(0.135\%)} & \multicolumn{1}{c|}{0.57(0\%)} & \multicolumn{1}{c|}{0.81(0\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.45\\(0.235\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Social\\Network}}} & \multicolumn{1}{c|}{0.48(0\%)} & \multicolumn{1}{c|}{0.34(0\%)} & \multicolumn{1}{c|}{\textbf{0.16(1.325\%)}} & \multicolumn{1}{c|}{0.58(0\%)} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{c|}{0(0.993\%)} & \multicolumn{1}{c|}{\textbf{0.51(2.318\%)}} & \multicolumn{1}{c|}{0.41(0\%)} & \multicolumn{1}{c|}{\textbf{0.13(2.649\%)}} & \multicolumn{1}{c|}{0.46(0\%)} & \multicolumn{1}{c|}{0.55(0\%)} & \multicolumn{1}{c|}{0.41(0.662\%)} & \multicolumn{1}{c|}{0.65(0\%)} & \multicolumn{1}{c|}{0.51(0.331\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.41\\(0.591\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Streaming}} & \multicolumn{1}{c|}{0.36(0.495\%)} & \multicolumn{1}{c|}{0.56(0.094\%)} & \multicolumn{1}{c|}{0.32(0.157\%)} & \multicolumn{1}{c|}{0.56(0.055\%)} & \multicolumn{1}{c|}{0.7(0.008\%)} & \multicolumn{1}{c|}{0.17(0.197\%)} & \multicolumn{1}{c|}{\textbf{0.49(0.967\%)}} & \multicolumn{1}{c|}{\textbf{0.46(0.605\%)}} & \multicolumn{1}{c|}{\textbf{0.21(0.873\%)}} & \multicolumn{1}{c|}{0.47(0.047\%)} & \multicolumn{1}{c|}{0.48(0.11\%)} & \multicolumn{1}{c|}{0.5(0.055\%)} & \multicolumn{1}{c|}{0.46(0.024\%)} & \multicolumn{1}{c|}{0.34(0.102\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.43\\(0.271\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Team\\management}}} & \multicolumn{1}{c|}{0.47(0.263\%)} & \multicolumn{1}{c|}{0.46(0.244\%)} & \multicolumn{1}{c|}{0.08(0.131\%)} & \multicolumn{1}{c|}{0.54(0.113\%)} & \multicolumn{1}{c|}{0.73(0\%)} & \multicolumn{1}{c|}{0.1(0.207\%)} & \multicolumn{1}{c|}{\textbf{0.44(0.976\%)}} & \multicolumn{1}{c|}{0.36(0\%)} & \multicolumn{1}{c|}{\textbf{0.16(8.092\%)}} & \multicolumn{1}{c|}{0.47(0\%)} & \multicolumn{1}{c|}{0.47(0.15\%)} & \multicolumn{1}{c|}{0.36(0.207\%)} & \multicolumn{1}{c|}{0.58(0\%)} & \multicolumn{1}{c|}{\textbf{0.12(0.676\%)}} & \multicolumn{1}{l|}{\textbf{\specialcell{0.38\\(0.79\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Tools}} & \multicolumn{1}{c|}{0.54(0.177\%)} & \multicolumn{1}{c|}{0.46(0.177\%)} & \multicolumn{1}{c|}{0.28(0.177\%)} & \multicolumn{1}{c|}{0.5(0.177\%)} & \multicolumn{1}{c|}{0.76(0\%)} & \multicolumn{1}{c|}{0.09(0.266\%)} & \multicolumn{1}{c|}{\textbf{0.5(1.329\%)}} & \multicolumn{1}{c|}{0.26(0.177\%)} & \multicolumn{1}{c|}{\textbf{0.34(0.531\%)}} & \multicolumn{1}{c|}{0.53(0\%)} & \multicolumn{1}{c|}{0.37(0.177\%)} & \multicolumn{1}{c|}{0.18(0.354\%)} & \multicolumn{1}{c|}{0.47(0.089\%)} & \multicolumn{1}{c|}{\textbf{0.31(2.303\%)}} & \multicolumn{1}{l|}{\textbf{\specialcell{0.4\\(0.424\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Tracking}} & \multicolumn{1}{c|}{0.46(0.102\%)} & \multicolumn{1}{c|}{0.59(0\%)} & \multicolumn{1}{c|}{0.1(0.43\%)} & \multicolumn{1}{c|}{0.51(0.02\%)} & \multicolumn{1}{c|}{0.69(0\%)} & \multicolumn{1}{c|}{\textbf{0.02(1.127\%)}} & \multicolumn{1}{c|}{\textbf{0.49(0.799\%)}} & \multicolumn{1}{c|}{0.23(0.061\%)} & \multicolumn{1}{c|}{0.34(0.656\%)} & \multicolumn{1}{c|}{0.39(0.102\%)} & \multicolumn{1}{c|}{0.39(0.41\%)} & \multicolumn{1}{c|}{0.36(0.184\%)} & \multicolumn{1}{c|}{0.48(0.348\%)} & \multicolumn{1}{c|}{\textbf{0.4(2.151\%)}} & \multicolumn{1}{l|}{\textbf{\specialcell{0.39\\(0.457\%)}}} \\ \midrule
    \multicolumn{1}{|l|}{\textbf{Training}} & \multicolumn{1}{c|}{0.2(0.239\%)} & \multicolumn{1}{c|}{0.57(0.032\%)} & \multicolumn{1}{c|}{0.11(0.239\%)} & \multicolumn{1}{c|}{0.52(0.026\%)} & \multicolumn{1}{c|}{0.71(0.006\%)} & \multicolumn{1}{c|}{0.17(0.355\%)} & \multicolumn{1}{c|}{\textbf{0.51(0.614\%)}} & \multicolumn{1}{c|}{0.42(0.032\%)} & \multicolumn{1}{c|}{0.4(0.491\%)} & \multicolumn{1}{c|}{0.49(0.026\%)} & \multicolumn{1}{c|}{0.25(0.071\%)} & \multicolumn{1}{c|}{\textbf{0.28(0.814\%)}} & \multicolumn{1}{c|}{\textbf{0.52(0.898\%)}} & \multicolumn{1}{c|}{0.44(0.071\%)} & \multicolumn{1}{l|}{\textbf{\specialcell{0.4\\(0.28\%)}}} \\ \midrule
\textbf{\specialcell{Grand\\Total}} & \textbf{\specialcell{0.47\\(0.197\%)}} & \textbf{\specialcell{0.55\\(0.042\%)}} & \textbf{\specialcell{0.18\\(0.418\%)}} & \textbf{\specialcell{0.54\\(0.08\%)}} & \textbf{\specialcell{0.54\\(0.033\%)}} & \textbf{\specialcell{0.18\\(0.377\%)}} & \textbf{\specialcell{0.48\\(1.282\%)}} & \textbf{\specialcell{0.45\\(0.112\%)}} & \textbf{\specialcell{0.27\\(1.165\%)}} & \textbf{\specialcell{0.35\\(0.381\%)}} & \textbf{\specialcell{0.42\\(0.087\%)}} & \textbf{\specialcell{0.33\\(0.798\%)}} & \textbf{\specialcell{0.51\\(0.21\%)}} & \textbf{\specialcell{0.36\\(0.339\%)}} & \textbf{\specialcell{0.4\\(0.394\%)}} \\ \bottomrule
\end{tabular}
}
\label{tab:sent-function-topic}
\end{sidewaystable}
%\end{table*}
%\end{adjustbox}


==> texfiles/images/senti-func-topic-updated-aug11.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

%\begin{table*}[!t]
\begin{sidewaystable}
%\begin{adjustbox}{angle=90} 
\centering
\small

\caption{Distribution of average review sentiment over different topics and different functionalities of sports apps. Also the percentage of negative sentiment reviews out of all reviews.} %\heng{all sentiment values are positive. the results are not quite helpful for answering the RQ: what are people complaining about? In addition to the average sentiment values, add the percentage of reviews with negative sentiment (what's the threshold used for tagging a negative sentiment, 0.05?). For example, put 10.23\% (0.20) where 10.23\% indicates the percentage of reviews of a app category and a topic that have negative sentiment, 0.20 indicate the average sentiment of all reviews of the app category and the topic.}
\label{tab:topic-function-senti}
\heng{for each app category, highlight the top three topics with highest percentage of reviews with negative sentiment}
%\heng{how to explain the positive feedback topic has the highest percentage of negative reviews? double check the result}
%\heng{here the grand total are for the sampled apps right? need a separate table for the topic sentiment of all 2,058 apps, similar to this table but only showing overall topic - sentiment (average sentiment and percentage of negative reviews). Then the grand total row can be removed from here (duplicated information).}\bhagya{I don't think it will be a duplicate information rather it shows the difference in distribution with the sample set and the whole dataset}\bhagya{updated rest of the comments}
\heng{similar comments as for Table 4: check the results }
\bhagya{updated}
\scalebox{0.48}{
\begin{tabular}{@{}|l|c|c|c|c|c|c|c|c|c|c|c|c|c|@{}}
\toprule
\textbf{Topic name} & \multicolumn{1}{l|}{\textbf{Betting}} & \multicolumn{1}{l|}{\textbf{Betting Tips}} & \multicolumn{1}{l|}{\textbf{Health Tips}} & \multicolumn{1}{l|}{\textbf{League Management}} & \multicolumn{1}{l|}{\textbf{Live updates}} & \multicolumn{1}{l|}{\textbf{News}} & \multicolumn{1}{l|}{\textbf{Radio}} & \multicolumn{1}{l|}{\textbf{Social Network}} & \multicolumn{1}{l|}{\textbf{Streaming}} & \multicolumn{1}{l|}{\textbf{Team management}} & \multicolumn{1}{l|}{\textbf{Tools}} & \multicolumn{1}{l|}{\textbf{Tracking}} & \multicolumn{1}{l|}{\textbf{Training}} \\ \midrule
\textbf{Accuracy of Models} & \textbf{0.13(17.89\%)} & \textbf{0.21(17.74\%)} & 0.39(7.17\%) & 0.27(0\%) & 0.42(6.48\%) & 0.37(7.23\%) & 0.33(6.12\%) & \textbf{0.42(14.29\%)} & 0.5(1.49\%) & 0.37(5.82\%) & 0.19(8.33\%) & 0.37(6.72\%) & 0.29(8.84\%) \\ \midrule
\textbf{Advertisement of UX} & 0.61(0\%) & 0.59(0.52\%) & 0.75(0\%) & 0.78(0\%) & 0.6(0.48\%) & 0.49(0.98\%) & 0.64(0\%) & 0.33(0\%) & \textbf{0.56(1.29\%)} & \textbf{0.46(3.23\%)} & \textbf{0.47(2.67\%)} & 0.59(0\%) & 0.57(1.81\%) \\ \midrule
\textbf{Bug reports} & 0(4.35\%) & 0.15(12.66\%) & 0.14(1.89\%) & 0.48(7.69\%) & 0.2(1.83\%) & 0.33(1.49\%) & 0.01(2.38\%) & 0.16(25\%) & 0.31(7.52\%) & \textbf{0.07(12.96\%)} & 0.29(7.14\%) & \textbf{0.1(19.63\%)} & \textbf{0.11(13.45\%)} \\ \midrule
\textbf{Feature Request} & 0.54(1.94\%) & 0.58(2.43\%) & \textbf{0.5(3.17\%)} & \textbf{0.51(10\%)} & 0.58(1.92\%) & 0.58(1.62\%) & 0.53(1.72\%) & 0.59(0\%) & \textbf{0.56(2.95\%)} & 0.54(1.6\%) & 0.5(2.17\%) & 0.51(0.39\%) & 0.52(0.8\%) \\ \midrule
\textbf{Impact of Application} & \textbf{0.53(1.59\%)} & 0.57(0\%) & 0.57(0\%) & 0.53(0\%) & \textbf{0.49(3.85\%)} & 0.44(1.53\%) & \textbf{0.37(1.15\%)} & 0.52(0\%) & 0.7(0.13\%) & 0.73(0\%) & 0.76(0\%) & 0.69(0\%) & 0.71(0.57\%) \\ \midrule
\textbf{Negative Feedback} & 0.2(3.26\%) & 0.15(8.21\%) & 0.09(15.19\%) & \textbf{0.03(25\%)} & 0.11(11.39\%) & 0.39(2.77\%) & 0.31(3.95\%) & \textbf{-0.01(20\%)} & 0.17(8.31\%) & 0.1(6.29\%) & 0.08(9.09\%) & \textbf{0.02(23.61\%)} & 0.17(5.41\%) \\ \midrule
\textbf{Positive Feedback} & \textbf{0.27(14.04\%)} & 0.34(6.88\%) & 0.47(4.1\%) & 0.49(2.75\%) & 0.57(1.61\%) & 0.54(2.39\%) & 0.47(5.31\%) & \textbf{0.51(7.95\%)} & 0.5(2.63\%) & 0.45(5.54\%) & \textbf{0.5(6.15\%)} & 0.5(4\%) & 0.52(1.76\%) \\ \midrule
\textbf{Precision of Tools} & 0.42(4\%) & 0.4(5.56\%) & 0.33(0\%) & 0.4(0\%) & 0.42(0\%) & 0.45(4.35\%) & \textbf{0.45(9.68\%)} & 0.45(0\%) & 0.46(3.37\%) & 0.37(0\%) & \textbf{0.26(11.76\%)} & \textbf{0.24(9.68\%)} & 0.42(7.25\%) \\ \midrule
\textbf{Quality of Content} & 0.55(2.91\%) & 0.52(2.83\%) & 0.52(0\%) & \textbf{0.49(7.14\%)} & 0.61(2.33\%) & 0.58(3.63\%) & \textbf{0.49(7.94\%)} & 0.48(0\%) & 0.36(5.67\%) & 0.47(4.15\%) & 0.54(4.17\%) & 0.46(5\%) & \textbf{0.2(18.59\%)} \\ \midrule
\textbf{Return on Investment} & 0.44(0\%) & 0.16(0.56\%) & 0.06(0\%) & 0.02(0\%) & 0.26(1.84\%) & 0.37(6.95\%) & 0.56(0\%) & 0.47(0\%) & 0.47(3.43\%) & 0.47(0\%) & 0.53(0\%) & \textbf{0.39(13.16\%)} & \textbf{0.5(5.19\%)} \\ \midrule
\textbf{Review credibility} & 0.48(2.22\%) & 0.47(1.34\%) & 0.56(0\%) & 0.62(0\%) & \textbf{0.45(2.97\%)} & 0.44(1.99\%) & 0.53(0\%) & 0.56(0\%) & \textbf{0.49(3.1\%)} & 0.47(2.71\%) & 0.38(1.53\%) & \textbf{0.4(3.39\%)} & 0.25(1.92\%) \\ \midrule
\textbf{Timeliness of updates} & 0.24(13.08\%) & 0.28(13.85\%) & 0.53(0\%) & 0.45(0\%) & \textbf{0.31(14.69\%)} & 0.43(6.82\%) & 0.81(0\%) & \textbf{0.51(14.29\%)} & 0.34(10.57\%) & \textbf{0.12(22.5\%)} & 0.32(9.52\%) & 0.41(7.62\%) & 0.44(6.32\%) \\ \midrule
\textbf{Version update} & 0.45(0\%) & \textbf{0.44(5.74\%)} & 0.45(3.7\%) & 0.4(0\%) & 0.46(3.64\%) & \textbf{0.43(8.57\%)} & 0.57(0\%) & 0.7(0\%) & 0.47(3.06\%) & 0.59(0\%) & \textbf{0.48(8.33\%)} & 0.48(4.96\%) & 0.53(3.34\%) \\ \midrule
\textbf{Video streaming quality} & 0.32(9.26\%) & 0.35(7.98\%) & 0.43(1.98\%) & 0.4(0\%) & 0.32(7.29\%) & 0.25(13.35\%) & 0.26(10.73\%) & \textbf{0.13(13.56\%)} & \textbf{0.22(13.42\%)} & \textbf{0.16(19.73\%)} & 0.35(7.06\%) & 0.35(7.49\%) & 0.41(6.5\%) \\ \bottomrule
\end{tabular}
}
\label{tab:sent-function-topic}
\end{sidewaystable}
%\end{table*}
%\end{adjustbox}


==> texfiles/images/sentiment-func-topic-updated.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table*}[!t]
\small
\caption{Distribution of average review sentiment over different topics and different functionalities of sports apps. Also the percentage of negative sentiment reviews out of all reviews. \heng{all sentiment values are positive. the results are not quite helpful for answering the RQ: what are people complaining about? In addition to the average sentiment values, add the percentage of reviews with negative sentiment (what's the threshold used for tagging a negative sentiment, 0.05?). For example, put 10.23\% (0.20) where 10.23\% indicates the percentage of reviews of a app category and a topic that have negative sentiment, 0.20 indicate the average sentiment of all reviews of the app category and the topic.}
\label{tab:topic-function-senti}
\heng{for each app category, highlight the top three topics with highest percentage of reviews with negative sentiment}}
\scalebox{0.325}{
\begin{tabular}{@{}|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|@{}}
\toprule
\textit{\textbf{Function}} & \multicolumn{1}{l|}{\textbf{\specialcell{Accuracy\\of Models}}} & \multicolumn{1}{l|}{\textbf{{\specialcell{Advertisement\\of UX}}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Bug\\reports}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Feature\\Request}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Impact\\of Application}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Negative\\Feedback}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Positive\\Feedback}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Precision\\of\\Tools}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Quality\\of\\Content}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Return\\on\\Investment}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Review\\credibility}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Timeliness\\of updates}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Version\\update}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Video\\streaming\\quality}}}& \textbf{\specialcell{Grand\\Total}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Betting}} & \multicolumn{1}{c|}{0.55(0.311\%)} & \multicolumn{1}{c|}{0.61(0\%)} & \multicolumn{1}{c|}{0(0.13\%)} & \multicolumn{1}{c|}{0.54(0.519\%)} & \multicolumn{1}{c|}{0.53(0.052\%)} & \multicolumn{1}{c|}{0.2(0.078\%)} & \multicolumn{1}{c|}{0.27(3.736\%)} & \multicolumn{1}{c|}{0.42(0.052\%)} & \multicolumn{1}{c|}{0.31(0.778\%)} & \multicolumn{1}{c|}{0.44(0\%)} & \multicolumn{1}{c|}{0.48(0.104\%)} & \multicolumn{1}{c|}{0.13(0.441\%)} & \multicolumn{1}{c|}{0.45(0\%)} & \multicolumn{1}{c|}{0.24(0.441\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.4\\(28.853\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Betting\\Tips}}} & \multicolumn{1}{c|}{0.52(0.241\%)} & \multicolumn{1}{c|}{0.59(0.008\%)} & \multicolumn{1}{c|}{0.15(1.932\%)} & \multicolumn{1}{c|}{0.57(0.084\%)} & \multicolumn{1}{c|}{0.56(0\%)} & \multicolumn{1}{c|}{0.15(0.414\%)} & \multicolumn{1}{c|}{0.34(3.112\%)} & \multicolumn{1}{c|}{0.39(0.015\%)} & \multicolumn{1}{c|}{0.35(0.414\%)} & \multicolumn{1}{c|}{0.16(0.008\%)} & \multicolumn{1}{c|}{0.47(0.031\%)} & \multicolumn{1}{c|}{0.21(2.637\%)} & \multicolumn{1}{c|}{0.44(0.054\%)} & \multicolumn{1}{c|}{0.28(0.245\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.3\\(40.046\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Health   Tips}} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{c|}{0.75(0\%)} & \multicolumn{1}{c|}{0.14(0.08\%)} & \multicolumn{1}{c|}{0.49(0.08\%)} & \multicolumn{1}{c|}{0.56(0\%)} & \multicolumn{1}{c|}{0.09(0.962\%)} & \multicolumn{1}{c|}{0.47(1.885\%)} & \multicolumn{1}{c|}{0.32(0\%)} & \multicolumn{1}{c|}{0.42(0.16\%)} & \multicolumn{1}{c|}{0.06(0\%)} & \multicolumn{1}{c|}{0.56(0\%)} & \multicolumn{1}{c|}{0.39(1.323\%)} & \multicolumn{1}{c|}{0.45(0.241\%)} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.41\\(25.862\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{League\\Management}}} & \multicolumn{1}{c|}{0.49(0.386\%)} & \multicolumn{1}{c|}{0.78(0\%)} & \multicolumn{1}{c|}{0.48(0.386\%)} & \multicolumn{1}{c|}{0.5(0.772\%)} & \multicolumn{1}{c|}{0.53(0\%)} & \multicolumn{1}{c|}{0.01(0.386\%)} & \multicolumn{1}{c|}{0.49(1.158\%)} & \multicolumn{1}{c|}{0.38(0\%)} & \multicolumn{1}{c|}{0.4(0\%)} & \multicolumn{1}{c|}{0.03(0\%)} & \multicolumn{1}{c|}{0.62(0\%)} & \multicolumn{1}{c|}{0.27(0\%)} & \multicolumn{1}{c|}{0.41(0\%)} & \multicolumn{1}{c|}{0.43(0\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.46\\(27.799\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Live\\updates}}} & \multicolumn{1}{c|}{0.61(0.065\%)} & \multicolumn{1}{c|}{0.6(0.007\%)} & \multicolumn{1}{c|}{0.2(0.08\%)} & \multicolumn{1}{c|}{0.58(0.065\%)} & \multicolumn{1}{c|}{0.49(0.065\%)} & \multicolumn{1}{c|}{0.11(0.567\%)} & \multicolumn{1}{c|}{0.57(0.771\%)} & \multicolumn{1}{c|}{0.42(0\%)} & \multicolumn{1}{c|}{0.32(0.625\%)} & \multicolumn{1}{c|}{0.26(0.138\%)} & \multicolumn{1}{c|}{0.44(0.058\%)} & \multicolumn{1}{c|}{0.42(0.778\%)} & \multicolumn{1}{c|}{0.45(0.029\%)} & \multicolumn{1}{c|}{0.31(0.262\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.46\\(25.645\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{News}} & \multicolumn{1}{c|}{0.58(0.159\%)} & \multicolumn{1}{c|}{0.49(0.023\%)} & \multicolumn{1}{c|}{0.33(0.061\%)} & \multicolumn{1}{c|}{0.58(0.045\%)} & \multicolumn{1}{c|}{0.44(0.03\%)} & \multicolumn{1}{c|}{0.39(0.144\%)} & \multicolumn{1}{c|}{0.54(0.605\%)} & \multicolumn{1}{c|}{0.44(0.038\%)} & \multicolumn{1}{c|}{0.25(1.286\%)} & \multicolumn{1}{c|}{0.37(2.292\%)} & \multicolumn{1}{c|}{0.44(0.045\%)} & \multicolumn{1}{c|}{0.37(0.34\%)} & \multicolumn{1}{c|}{0.43(0.068\%)} & \multicolumn{1}{c|}{0.43(0.182\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.43\\(23.839\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Radio}} & \multicolumn{1}{c|}{0.5(0.225\%)} & \multicolumn{1}{c|}{0.64(0\%)} & \multicolumn{1}{c|}{0.01(0.045\%)} & \multicolumn{1}{c|}{0.53(0.045\%)} & \multicolumn{1}{c|}{0.37(0.54\%)} & \multicolumn{1}{c|}{0.31(0.135\%)} & \multicolumn{1}{c|}{0.46(0.9\%)} & \multicolumn{1}{c|}{0.45(0.135\%)} & \multicolumn{1}{c|}{0.26(1.125\%)} & \multicolumn{1}{c|}{0.58(0\%)} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{c|}{0.33(0.135\%)} & \multicolumn{1}{c|}{0.57(0\%)} & \multicolumn{1}{c|}{0.81(0\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.4\\(33.753\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Social\\Network}}} & \multicolumn{1}{c|}{0.48(0\%)} & \multicolumn{1}{c|}{0.34(0\%)} & \multicolumn{1}{c|}{0.16(1.325\%)} & \multicolumn{1}{c|}{0.58(0\%)} & \multicolumn{1}{c|}{0.52(0\%)} & \multicolumn{1}{c|}{0(0.993\%)} & \multicolumn{1}{c|}{0.51(2.318\%)} & \multicolumn{1}{c|}{0.41(0\%)} & \multicolumn{1}{c|}{0.13(2.649\%)} & \multicolumn{1}{c|}{0.46(0\%)} & \multicolumn{1}{c|}{0.55(0\%)} & \multicolumn{1}{c|}{0.41(0.662\%)} & \multicolumn{1}{c|}{0.65(0\%)} & \multicolumn{1}{c|}{0.51(0.331\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.38\\(28.146\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Streaming}} & \multicolumn{1}{c|}{0.36(0.495\%)} & \multicolumn{1}{c|}{0.56(0.094\%)} & \multicolumn{1}{c|}{0.32(0.157\%)} & \multicolumn{1}{c|}{0.56(0.055\%)} & \multicolumn{1}{c|}{0.7(0.008\%)} & \multicolumn{1}{c|}{0.17(0.197\%)} & \multicolumn{1}{c|}{0.49(0.967\%)} & \multicolumn{1}{c|}{0.46(0.605\%)} & \multicolumn{1}{c|}{0.21(0.873\%)} & \multicolumn{1}{c|}{0.47(0.047\%)} & \multicolumn{1}{c|}{0.48(0.11\%)} & \multicolumn{1}{c|}{0.5(0.055\%)} & \multicolumn{1}{c|}{0.46(0.024\%)} & \multicolumn{1}{c|}{0.34(0.102\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.46\\(23.652\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{\specialcell{Team\\management}}} & \multicolumn{1}{c|}{0.47(0.263\%)} & \multicolumn{1}{c|}{0.46(0.244\%)} & \multicolumn{1}{c|}{0.08(0.131\%)} & \multicolumn{1}{c|}{0.54(0.113\%)} & \multicolumn{1}{c|}{0.73(0\%)} & \multicolumn{1}{c|}{0.1(0.207\%)} & \multicolumn{1}{c|}{0.44(0.976\%)} & \multicolumn{1}{c|}{0.36(0\%)} & \multicolumn{1}{c|}{0.16(8.092\%)} & \multicolumn{1}{c|}{0.47(0\%)} & \multicolumn{1}{c|}{0.47(0.15\%)} & \multicolumn{1}{c|}{0.36(0.207\%)} & \multicolumn{1}{c|}{0.58(0\%)} & \multicolumn{1}{c|}{0.12(0.676\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.32\\(29.835\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Tools}} & \multicolumn{1}{c|}{0.54(0.177\%)} & \multicolumn{1}{c|}{0.46(0.177\%)} & \multicolumn{1}{c|}{0.28(0.177\%)} & \multicolumn{1}{c|}{0.5(0.177\%)} & \multicolumn{1}{c|}{0.76(0\%)} & \multicolumn{1}{c|}{0.09(0.266\%)} & \multicolumn{1}{c|}{0.5(1.329\%)} & \multicolumn{1}{c|}{0.26(0.177\%)} & \multicolumn{1}{c|}{0.34(0.531\%)} & \multicolumn{1}{c|}{0.53(0\%)} & \multicolumn{1}{c|}{0.37(0.177\%)} & \multicolumn{1}{c|}{0.18(0.354\%)} & \multicolumn{1}{c|}{0.47(0.089\%)} & \multicolumn{1}{c|}{0.31(2.303\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.4\\(25.686\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Tracking}} & \multicolumn{1}{c|}{0.46(0.102\%)} & \multicolumn{1}{c|}{0.59(0\%)} & \multicolumn{1}{c|}{0.1(0.43\%)} & \multicolumn{1}{c|}{0.51(0.02\%)} & \multicolumn{1}{c|}{0.69(0\%)} & \multicolumn{1}{c|}{0.02(1.127\%)} & \multicolumn{1}{c|}{0.49(0.799\%)} & \multicolumn{1}{c|}{0.23(0.061\%)} & \multicolumn{1}{c|}{0.34(0.656\%)} & \multicolumn{1}{c|}{0.39(0.102\%)} & \multicolumn{1}{c|}{0.39(0.41\%)} & \multicolumn{1}{c|}{0.36(0.184\%)} & \multicolumn{1}{c|}{0.48(0.348\%)} & \multicolumn{1}{c|}{0.4(2.151\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.41\\(24.134\%)}}} \\ \midrule
\multicolumn{1}{|l|}{\textbf{Training}} & \multicolumn{1}{c|}{0.2(0.239\%)} & \multicolumn{1}{c|}{0.57(0.032\%)} & \multicolumn{1}{c|}{0.11(0.239\%)} & \multicolumn{1}{c|}{0.52(0.026\%)} & \multicolumn{1}{c|}{0.71(0.006\%)} & \multicolumn{1}{c|}{0.17(0.355\%)} & \multicolumn{1}{c|}{0.51(0.614\%)} & \multicolumn{1}{c|}{0.42(0.032\%)} & \multicolumn{1}{c|}{0.4(0.491\%)} & \multicolumn{1}{c|}{0.49(0.026\%)} & \multicolumn{1}{c|}{0.25(0.071\%)} & \multicolumn{1}{c|}{0.28(0.814\%)} & \multicolumn{1}{c|}{0.52(0.898\%)} & \multicolumn{1}{c|}{0.44(0.071\%)} & \multicolumn{1}{c|}{\textbf{\specialcell{0.45\\(25.757\%)}}} \\ \midrule
\textbf{\specialcell{Grand\\Total}} & \textbf{\specialcell{0.47\\(0.197\%)}} & \textbf{\specialcell{0.55\\(0.042\%)}} & \textbf{\specialcell{0.18\\(0.418\%)}} & \textbf{\specialcell{0.54\\(0.08\%)}} & \textbf{\specialcell{0.54\\(0.033\%)}} & \textbf{\specialcell{0.18\\(0.377\%)}} & \textbf{\specialcell{0.48\\(1.282\%)}} & \textbf{\specialcell{0.45\\(0.112\%)}} & \textbf{\specialcell{0.27\\(1.165\%)}} & \textbf{\specialcell{0.35\\(0.381\%)}} & \textbf{\specialcell{0.42\\(0.087\%)}} & \textbf{\specialcell{0.33\\(0.798\%)}} & \textbf{\specialcell{0.51\\(0.21\%)}} & \textbf{\specialcell{0.36\\(0.339\%)}} & \textbf{} \\ \bottomrule
\end{tabular}}
\label{tab:sent-function-topic}
\end{table*}


==> texfiles/images/sentiment-function-topic.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table*}[!t]
\small
\caption{Distribution of average review sentiment over different topics and different functionalities of sports apps. Also the percentage of negative sentiment reviews out of all reviews. \heng{all sentiment values are positive. the results are not quite helpful for answering the RQ: what are people complaining about? In addition to the average sentiment values, add the percentage of reviews with negative sentiment (what's the threshold used for tagging a negative sentiment, 0.05?). For example, put 10.23\% (0.20) where 10.23\% indicates the percentage of reviews of a app category and a topic that have negative sentiment, 0.20 indicate the average sentiment of all reviews of the app category and the topic.}
\label{tab:topic-function-senti}
\heng{for each app category, highlight the top three topics with highest percentage of reviews with negative sentiment}}
\scalebox{0.32}{
\begin{tabular}{@{}|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|@{}}
\toprule
\textit{\textbf{Function}} & \multicolumn{1}{l|}{\textbf{\specialcell{Accuracy\\of Models}}} & \multicolumn{1}{l|}{\textbf{{\specialcell{Advertisement\\of UX}}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Bug\\reports}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Feature\\Request}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Impact\\of Application}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Negative\\Feedback}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Positive\\Feedback}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Precision\\of\\Tools}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Quality\\of\\Content}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Return\\on\\Investment}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Review\\credibility}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Timeliness\\of updates}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Version\\update}}} & \multicolumn{1}{l|}{\textbf{\specialcell{Video\\streaming\\quality}}} \\ \midrule
\textbf{Betting} & 0.55(0.311\%) & 0.61(0\%) & 0(0.13\%) & 0.54(0.519\%) & 0.53(0.052\%) & 0.2(0.078\%) & 0.27(3.736\%) & 0.42(0.052\%) & 0.31(0.778\%) & 0.44(0\%) & 0.48(0.104\%) & 0.13(0.441\%) & 0.45(0\%) & 0.24(0.441\%) \\ \midrule
\textbf{\specialcell{Betting\\Tips}} & 0.52(0.241\%) & 0.59(0.008\%) & 0.15(1.932\%) & 0.57(0.084\%) & 0.56(0\%) & 0.15(0.414\%) & 0.34(3.112\%) & 0.39(0.015\%) & 0.35(0.414\%) & 0.16(0.008\%) & 0.47(0.031\%) & 0.21(2.637\%) & 0.44(0.054\%) & 0.28(0.245\%) \\ \midrule
\textbf{\specialcell{Health\\Tips}} & 0.52(0\%) & 0.75(0\%) & 0.14(0.08\%) & 0.49(0.08\%) & 0.56(0\%) & 0.09(0.962\%) & 0.47(1.885\%) & 0.32(0\%) & 0.42(0.16\%) & 0.06(0\%) & 0.56(0\%) & 0.39(1.323\%) & 0.45(0.241\%) & 0.52(0\%) \\ \midrule
\textbf{\specialcell{League\\ Management}} & 0.49(0.386\%) & 0.78(0\%) & 0.48(0.386\%) & 0.5(0.772\%) & 0.53(0\%) & 0.01(0.386\%) & 0.49(1.158\%) & 0.38(0\%) & 0.4(0\%) & 0.03(0\%) & 0.62(0\%) & 0.27(0\%) & 0.41(0\%) & 0.43(0\%) \\ \midrule
\textbf{\specialcell{Live\\updates}} & 0.61(0.065\%) & 0.6(0.007\%) & 0.2(0.08\%) & 0.58(0.065\%) & 0.49(0.065\%) & 0.11(0.567\%) & 0.57(0.771\%) & 0.42(0\%) & 0.32(0.625\%) & 0.26(0.138\%) & 0.44(0.058\%) & 0.42(0.778\%) & 0.45(0.029\%) & 0.31(0.262\%) \\ \midrule
\textbf{News} & 0.58(0.159\%) & 0.49(0.023\%) & 0.33(0.061\%) & 0.58(0.045\%) & 0.44(0.03\%) & 0.39(0.144\%) & 0.54(0.605\%) & 0.44(0.038\%) & 0.25(1.286\%) & 0.37(2.292\%) & 0.44(0.045\%) & 0.37(0.34\%) & 0.43(0.068\%) & 0.43(0.182\%) \\ \midrule
\textbf{Radio} & 0.5(0.225\%) & 0.64(0\%) & 0.01(0.045\%) & 0.53(0.045\%) & 0.37(0.54\%) & 0.31(0.135\%) & 0.46(0.9\%) & 0.45(0.135\%) & 0.26(1.125\%) & 0.58(0\%) & 0.52(0\%) & 0.33(0.135\%) & 0.57(0\%) & 0.81(0\%) \\ \midrule
\textbf{\specialcell{Social\\Network}} & 0.48(0\%) & 0.34(0\%) & 0.16(1.325\%) & 0.58(0\%) & 0.52(0\%) & 0(0.993\%) & 0.51(2.318\%) & 0.41(0\%) & 0.13(2.649\%) & 0.46(0\%) & 0.55(0\%) & 0.41(0.662\%) & 0.65(0\%) & 0.51(0.331\%) \\ \midrule
\textbf{Streaming} & 0.36(0.495\%) & 0.56(0.094\%) & 0.32(0.157\%) & 0.56(0.055\%) & 0.7(0.008\%) & 0.17(0.197\%) & 0.49(0.967\%) & 0.46(0.605\%) & 0.21(0.873\%) & 0.47(0.047\%) & 0.48(0.11\%) & 0.5(0.055\%) & 0.46(0.024\%) & 0.34(0.102\%) \\ \midrule
\textbf{\specialcell{Team\\management}} & 0.47(0.263\%) & 0.46(0.244\%) & 0.08(0.131\%) & 0.54(0.113\%) & 0.73(0\%) & 0.1(0.207\%) & 0.44(0.976\%) & 0.36(0\%) & 0.16(8.092\%) & 0.47(0\%) & 0.47(0.15\%) & 0.36(0.207\%) & 0.58(0\%) & 0.12(0.676\%) \\ \midrule
\textbf{Tools} & 0.54(0.177\%) & 0.46(0.177\%) & 0.28(0.177\%) & 0.5(0.177\%) & 0.76(0\%) & 0.09(0.266\%) & 0.5(1.329\%) & 0.26(0.177\%) & 0.34(0.531\%) & 0.53(0\%) & 0.37(0.177\%) & 0.18(0.354\%) & 0.47(0.089\%) & 0.31(2.303\%) \\ \midrule
\textbf{Tracking} & 0.46(0.102\%) & 0.59(0\%) & 0.1(0.43\%) & 0.51(0.02\%) & 0.69(0\%) & 0.02(1.127\%) & 0.49(0.799\%) & 0.23(0.061\%) & 0.34(0.656\%) & 0.39(0.102\%) & 0.39(0.41\%) & 0.36(0.184\%) & 0.48(0.348\%) & 0.4(2.151\%) \\ \midrule
\textbf{Training} & 0.2(0.239\%) & 0.57(0.032\%) & 0.11(0.239\%) & 0.52(0.026\%) & 0.71(0.006\%) & 0.17(0.355\%) & 0.51(0.614\%) & 0.42(0.032\%) & 0.4(0.491\%) & 0.49(0.026\%) & 0.25(0.071\%) & 0.28(0.814\%) & 0.52(0.898\%) & 0.44(0.071\%) \\ \midrule
\textbf{\specialcell{Grand\\Total}} & \textbf{0.47(0.197\%)} & \textbf{0.55(0.042\%)} & \textbf{0.18(0.418\%)} & \textbf{0.54(0.08\%)} & \textbf{0.54(0.033\%)} & \textbf{0.18(0.377\%)} & \textbf{0.48(1.282\%)} & \textbf{0.45(0.112\%)} & \textbf{0.27(1.165\%)} & \textbf{0.35(0.381\%)} & \textbf{0.42(0.087\%)} & \textbf{0.33(0.798\%)} & \textbf{0.51(0.21\%)} & \textbf{0.36(0.339\%)} \\ \bottomrule
\end{tabular}}
\label{tab:sent-function-topic}
\end{table*}


==> texfiles/images/sentiment-topic-functions.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}

\begin{table*}[!t]
\small
\caption{Distribution of average review sentiment over different topics and different functionalities of sports apps. Also the percentage of negative sentiment reviews out of all reviews. \heng{all sentiment values are positive. the results are not quite helpful for answering the RQ: what are people complaining about? In addition to the average sentiment values, add the percentage of reviews with negative sentiment (what's the threshold used for tagging a negative sentiment, 0.05?). For example, put 10.23\% (0.20) where 10.23\% indicates the percentage of reviews of a app category and a topic that have negative sentiment, 0.20 indicate the average sentiment of all reviews of the app category and the topic.}
\label{tab:topic-function-senti}
\heng{for each app category, highlight the top three topics with highest percentage of reviews with negative sentiment}}
\scalebox{0.32}{
\begin{tabular}{@{}|l|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|@{}}
\toprule
\textit{\textbf{Function}} & \multicolumn{1}{l|}{\textbf{Accuracy   of Models}} & \multicolumn{1}{l|}{\textbf{Advertisement   of UX}} & \multicolumn{1}{l|}{\textbf{Bug   reports}} & \multicolumn{1}{l|}{\textbf{Feature   Request}} & \multicolumn{1}{l|}{\textbf{Impact   of Application}} & \multicolumn{1}{l|}{\textbf{Negative   Feedback}} & \multicolumn{1}{l|}{\textbf{Positive   Feedback}} & \multicolumn{1}{l|}{\textbf{Precision   of Tools}} & \multicolumn{1}{l|}{\textbf{Quality   of Content}} & \multicolumn{1}{l|}{\textbf{Return   on Investment}} & \multicolumn{1}{l|}{\textbf{Review   credibility}} & \multicolumn{1}{l|}{\textbf{Timeliness   of updates}} & \multicolumn{1}{l|}{\textbf{Version   update}} & \multicolumn{1}{l|}{\textbf{Video   streaming quality}} & \textbf{Grand Total} \\ \midrule
\textbf{Betting} & 0.55(0.311\%) & 0.61(0\%) & 0(0.13\%) & 0.54(0.519\%) & 0.53(0.052\%) & 0.2(0.078\%) & 0.27(3.736\%) & 0.42(0.052\%) & 0.31(0.778\%) & 0.44(0\%) & 0.48(0.104\%) & 0.13(0.441\%) & 0.45(0\%) & 0.24(0.441\%) & \textbf{0.4(28.853\%)} \\ \midrule
\textbf{Betting   Tips} & 0.52(0.241\%) & 0.59(0.008\%) & 0.15(1.932\%) & 0.57(0.084\%) & 0.56(0\%) & 0.15(0.414\%) & 0.34(3.112\%) & 0.39(0.015\%) & 0.35(0.414\%) & 0.16(0.008\%) & 0.47(0.031\%) & 0.21(2.637\%) & 0.44(0.054\%) & 0.28(0.245\%) & \textbf{0.3(40.046\%)} \\ \midrule
\textbf{Health   Tips} & 0.52(0\%) & 0.75(0\%) & 0.14(0.08\%) & 0.49(0.08\%) & 0.56(0\%) & 0.09(0.962\%) & 0.47(1.885\%) & 0.32(0\%) & 0.42(0.16\%) & 0.06(0\%) & 0.56(0\%) & 0.39(1.323\%) & 0.45(0.241\%) & 0.52(0\%) & \textbf{0.41(25.862\%)} \\ \midrule
\textbf{League   Management} & 0.49(0.386\%) & 0.78(0\%) & 0.48(0.386\%) & 0.5(0.772\%) & 0.53(0\%) & 0.01(0.386\%) & 0.49(1.158\%) & 0.38(0\%) & 0.4(0\%) & 0.03(0\%) & 0.62(0\%) & 0.27(0\%) & 0.41(0\%) & 0.43(0\%) & \textbf{0.46(27.799\%)} \\ \midrule
\textbf{Live   updates} & 0.61(0.065\%) & 0.6(0.007\%) & 0.2(0.08\%) & 0.58(0.065\%) & 0.49(0.065\%) & 0.11(0.567\%) & 0.57(0.771\%) & 0.42(0\%) & 0.32(0.625\%) & 0.26(0.138\%) & 0.44(0.058\%) & 0.42(0.778\%) & 0.45(0.029\%) & 0.31(0.262\%) & \textbf{0.46(25.645\%)} \\ \midrule
\textbf{News} & 0.58(0.159\%) & 0.49(0.023\%) & 0.33(0.061\%) & 0.58(0.045\%) & 0.44(0.03\%) & 0.39(0.144\%) & 0.54(0.605\%) & 0.44(0.038\%) & 0.25(1.286\%) & 0.37(2.292\%) & 0.44(0.045\%) & 0.37(0.34\%) & 0.43(0.068\%) & 0.43(0.182\%) & \textbf{0.43(23.839\%)} \\ \midrule
\textbf{Radio} & 0.5(0.225\%) & 0.64(0\%) & 0.01(0.045\%) & 0.53(0.045\%) & 0.37(0.54\%) & 0.31(0.135\%) & 0.46(0.9\%) & 0.45(0.135\%) & 0.26(1.125\%) & 0.58(0\%) & 0.52(0\%) & 0.33(0.135\%) & 0.57(0\%) & 0.81(0\%) & \textbf{0.4(33.753\%)} \\ \midrule
\textbf{Social   Network} & 0.48(0\%) & 0.34(0\%) & 0.16(1.325\%) & 0.58(0\%) & 0.52(0\%) & 0(0.993\%) & 0.51(2.318\%) & 0.41(0\%) & 0.13(2.649\%) & 0.46(0\%) & 0.55(0\%) & 0.41(0.662\%) & 0.65(0\%) & 0.51(0.331\%) & \textbf{0.38(28.146\%)} \\ \midrule
\textbf{Streaming} & 0.36(0.495\%) & 0.56(0.094\%) & 0.32(0.157\%) & 0.56(0.055\%) & 0.7(0.008\%) & 0.17(0.197\%) & 0.49(0.967\%) & 0.46(0.605\%) & 0.21(0.873\%) & 0.47(0.047\%) & 0.48(0.11\%) & 0.5(0.055\%) & 0.46(0.024\%) & 0.34(0.102\%) & \textbf{0.46(23.652\%)} \\ \midrule
\textbf{Team   management} & 0.47(0.263\%) & 0.46(0.244\%) & 0.08(0.131\%) & 0.54(0.113\%) & 0.73(0\%) & 0.1(0.207\%) & 0.44(0.976\%) & 0.36(0\%) & 0.16(8.092\%) & 0.47(0\%) & 0.47(0.15\%) & 0.36(0.207\%) & 0.58(0\%) & 0.12(0.676\%) & \textbf{0.32(29.835\%)} \\ \midrule
\textbf{Tools} & 0.54(0.177\%) & 0.46(0.177\%) & 0.28(0.177\%) & 0.5(0.177\%) & 0.76(0\%) & 0.09(0.266\%) & 0.5(1.329\%) & 0.26(0.177\%) & 0.34(0.531\%) & 0.53(0\%) & 0.37(0.177\%) & 0.18(0.354\%) & 0.47(0.089\%) & 0.31(2.303\%) & \textbf{0.4(25.686\%)} \\ \midrule
\textbf{Tracking} & 0.46(0.102\%) & 0.59(0\%) & 0.1(0.43\%) & 0.51(0.02\%) & 0.69(0\%) & 0.02(1.127\%) & 0.49(0.799\%) & 0.23(0.061\%) & 0.34(0.656\%) & 0.39(0.102\%) & 0.39(0.41\%) & 0.36(0.184\%) & 0.48(0.348\%) & 0.4(2.151\%) & \textbf{0.41(24.134\%)} \\ \midrule
\textbf{Training} & 0.2(0.239\%) & 0.57(0.032\%) & 0.11(0.239\%) & 0.52(0.026\%) & 0.71(0.006\%) & 0.17(0.355\%) & 0.51(0.614\%) & 0.42(0.032\%) & 0.4(0.491\%) & 0.49(0.026\%) & 0.25(0.071\%) & 0.28(0.814\%) & 0.52(0.898\%) & 0.44(0.071\%) & \textbf{0.45(25.757\%)} \\ \midrule
\textbf{Grand   Total} & \textbf{0.47(0.197\%)} & \textbf{0.55(0.042\%)} & \textbf{0.18(0.418\%)} & \textbf{0.54(0.08\%)} & \textbf{0.54(0.033\%)} & \textbf{0.18(0.377\%)} & \textbf{0.48(1.282\%)} & \textbf{0.45(0.112\%)} & \textbf{0.27(1.165\%)} & \textbf{0.35(0.381\%)} & \textbf{0.42(0.087\%)} & \textbf{0.33(0.798\%)} & \textbf{0.51(0.21\%)} & \textbf{0.36(0.339\%)} & \textbf{} \\ \bottomrule
\end{tabular}}
\label{tab:sent-function-topic}
\end{table*}


==> texfiles/images/topic-function-table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{sidewaystable}
% \begin{sidewaystabe}[!t]
% \begin{table*}[!t]
% \tiny
% \label{topic-function}
\caption{Distribution of different topics among different functionalities of sports apps.\heng{The results look strange: why the most frequent topic of radio apps is impact of application? why the most frequent topic of team management is quality of content? why video streaming quality for tools and tracking (the video streaming quality has only 0.96\% for streaming apps!)? Double check the results.}\bhagya{I have double checked the results and added explanation for why it happened on the confusing metrics}
\label{tab:topic-function}
\heng{highlight the top three topics for each app category}}
\scalebox{0.6}{
\begin{tabular}{@{}|l|r|r|r|r|r|r|r|r|r|r|r|r|r|r|@{}}
\toprule
\textit{\textbf{Function}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Positive\\Feedback}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Quality of\\Content}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Version\\update}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{up-to-\\dateness}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Return on\\Investment}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Negative\\Feedback}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Video\\streaming\\quality}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Review\\credibility}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Precision of\\Tools}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Accuracy of\\Prediction}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Adverti-\\sement}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Impact of\\Application}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Feature\\Request}}} &
  \multicolumn{1}{l|}{\textbf{\specialcell{Bug\\reports}}} \\ \midrule
\textbf{Betting} &
  \textbf{29.12\%} &
  7.71\% &
  0.96\% &
  2.57\% &
  0.85\% &
  2.10\% &
  2.85\% &
  3.97\% &
  0.97\% &
  \textbf{15.52\%} &
  4.52\% &
  3.02\% &
  \textbf{23.24\%} &
  2.61\% \\ \midrule
\textbf{Betting Tips} &
  \textbf{46.71\%} &
  4.95\% &
  0.84\% &
  \textbf{15.37\%} &
  1.33\% &
  5.07\% &
  1.65\% &
  2.21\% &
  0.28\% &
  1.46\% &
  1.38\% &
  1.10\% &
  3.26\% &
  \textbf{14.40\%}\\ \midrule
\textbf{Health Tips} &
  \textbf{46.67\%} &
  \textbf{8.02\%} &
  6.20\% &
  \textbf{18.55\%} &
  1.65\% &
  6.33\% &
  0.77\% &
  2.46\% &
  0.16\% &
  0.89\% &
  0.77\% &
  0.96\% &
  2.45\% &
  4.12\% \\ \midrule
\textbf{League Management} &
  \textbf{42.12\%} &
  \textbf{10.03\%} &
  1.16\% &
  5.04\% &
  5.02\% &
  1.55\% &
  3.85\% &
  5.01\% &
  0.77\% &
  5.40\% &
  4.63\% &
  2.70\% &
  \textbf{7.71\%} &
  5.01\% \\ \midrule
\textbf{Live updates} &
  \textbf{49.65\%} &
  \textbf{8.46\%} &
  0.78\% &
  \textbf{12.09\%} &
  6.84\% &
  4.88\% &
  1.68\% &
  1.88\% &
  0.65\% &
  2.51\% &
  1.48\% &
  1.64\% &
  3.33\% &
  4.13\% \\ \midrule
\textbf{News} &
  \textbf{26.42\%} &
  \textbf{9.64\%} &
  0.80\% &
  4.93\% &
  \textbf{32.11\%} &
  5.35\% &
  2.58\% &
  2.27\% &
  0.85\% &
  4.15\% &
  2.21\% &
  1.94\% &
  2.75\% &
  4.01\% \\ \midrule
\textbf{Radio} &
  \textbf{17.01\%} &
  \textbf{10.52\%} &
  0.45\% &
  2.21\% &
  0.77\% &
  3.44\% &
  1.35\% &
  3.97\% &
  1.40\% &
  2.83\% &
  4.69\% &
  \textbf{46.87\%} &
  2.61\% &
  1.89\% \\ \midrule
\textbf{Social Network} &
  \textbf{29.16\%} &
  \textbf{19.52\%} &
  0.33\% &
  4.64\% &
  \textbf{7.94\%} &
  4.96\% &
  2.32\% &
  6.62\% &
  0.66\% &
  5.96\% &
  4.97\% &
  3.98\% &
  3.64\% &
  5.30\% \\ \midrule
\textbf{Streaming} &
  \textbf{36.06\%} &
  6.35\% &
  0.75\% &
  3.57\% &
  1.34\% &
  2.29\% &
  0.96\% &
  3.54\% &
  \textbf{18.98\%} &
  \textbf{8.79\%} &
  7.59\% &
  5.87\% &
  1.86\% &
  2.05\% \\ \midrule
\textbf{Team management} &
  \textbf{17.76\%} &
  \textbf{40.94\%} &
  0.58\% &
  3.58\% &
  0.51\% &
  3.32\% &
  3.01\% &
  5.50\% &
  0.45\% &
  6.27\% &
  \textbf{7.49\%} &
  2.53\% &
  7.04\% &
  1.01\% \\ \midrule
\textbf{Tools} &
  \textbf{21.65\%} &
  7.54\% &
  1.07\% &
  4.26\% &
  1.95\% &
  2.93\% &
  \textbf{24.12\%} &
  \textbf{11.58\%} &
  1.51\% &
  4.26\% &
  6.64\% &
  1.86\% &
  8.16\% &
  2.48\% \\ \midrule
\textbf{Tracking} &
  \textbf{20.05\%} &
  \textbf{8.74\%} &
  7.15\% &
  2.76\% &
  0.78\% &
  4.75\% &
  \textbf{28.09\%} &
  12.04\% &
  0.64\% &
  2.05\% &
  3.48\% &
  2.04\% &
  5.23\% &
  2.19\% \\ \midrule
\textbf{Training} &
  \textbf{35.49\%} &
  7.63\% &
  \textbf{26.25\%} &
  \textbf{9.40\% }&
  0.49\% &
  6.64\% &
  1.09\% &
  3.59\% &
  0.43\% &
  1.24\% &
  1.75\% &
  1.11\% &
  3.13\% &
  1.74\% \\ \midrule
\textbf{Grand Total} &
  \textbf{32.50\%} &
  \textbf{10.79\%} &
  \textbf{9.50\%} &
  \textbf{6.89\%} &
  \textbf{5.62\%} &
  \textbf{4.83\%} &
  \textbf{4.34\%} &
  \textbf{4.28\%} &
  \textbf{3.90\%} &
  \textbf{3.77\%} &
  \textbf{3.66\%} &
  \textbf{3.59\%} &
  \textbf{3.52\%} &
  \textbf{2.80\%} \\ \bottomrule
\end{tabular}
}
\end{sidewaystable}
% \end{table*}



==> texfiles/keywords-table.tex <==
\label{table:yake-keyword}
\begin{table}
\caption{Keyword Extraction by YAKE. \heng{The table is not necessary and it's a waste of space. The score does not provide any thing valuable. List the keywords in a more compact table or simply list them in the text at the appripriate place.}}
\label{tab:conf}
\begin{minipage}{\columnwidth}
\begin{center}
\begin{tabular}{c| c}

\textbf{Yake Keywords} & \textbf{Yake score}\\ \midrule
\toprule


golf GPS &	2.11E-04 \\
sports betting	& 1.99E-04 \\
sports betting tips &	1.97E-04 \\
soccer betting &	1.89E-04\\
fitivity &	1.85E-04\\
fitness	& 1.83E-04\\
football betting tips &	1.83E-04\\
soccer training &	1.81E-04\\
sports leauges &	1.75E-04\\
football tips  &	1.68E-04\\
NBA League Pass	 & 1.63E-04\\
Fitivity Premium subscription &	1.46E-04\\
Live Sports &	1.37E-04\\
sports network Live & 	1.37E-04 \\
Pro sports subscription &	1.11E-04 \\
State football & 	1.09E-04 \\
football training & 	9.68E-05 \\
champions league &	5.12E-05 \\
premier league &	3.12E-05 \\
sports player &	7.56E-06 \\
\bottomrule
\end{tabular}
\end{center}
\bigskip


\end{minipage}
\end{table}

==> texfiles/methodology.tex <==
\section{Methodology} \label{sec:method}

\heng{Move the content of this section to Section~\ref{sec:setup} and the approach parts of Section~\ref{sec:results}, following the suggested structures in the two sections}. 

This section summarises the approaches we used to extract and analyze the sports app data and address the research questions mentioned.
\newline

\subsection{Scraping sports-related apps from the Google Play store}

\textbf{Preparing the dataset}
\newline
Google Play store provided tags for each application. But from our primary analysis, we understood that developers placing their app in the play store does not pay much attention to the tags available, thus making it tedious to extract. To identify sports apps from all the other apps, we need to have a set of keywords that we can use as the search keywords 
\newline The approach we used to generate those keywords are as follow
 
1)\textbf { Top-rated sports apps from AppBrain:} AppBrain will provide the details about app categories, and we downloaded top-rated apps in the US. From the dataset, we analyzed the following metadata: Google Play URL, Short description, Launch time, Last update time, Rating, Comment count. We used this as our reference set, and we used the Google Play URL to get a detailed description of these apps for our next step. We also decided to avoid games from our list of apps (specifically keyword games and fantasy games) as those are not sports apps for our problem definition.
 
2) \textbf{Finding keywords for iterative search:} Google Play store also limits the list retrieved per request to 250 for each query. So we had to find a list of keywords to run iterative queries, extract a maximum number of apps, and remove the duplicates. We looked into the title and description of the top-rated sports apps and applied keywords extraction algorithm YAKE [9] with a window size of 3 and used these keywords for further iterative search and extracted apps related to the keywords.
\newline The extracted keywords underwent a manual analysis for affirming the selection. The final keyword list was 20 keywords (Fig 1). According to YAKE documentation the lower the score the more relevant the keyword is.

We did the iterative extraction of apps with these keywords, and our final dataset was 3072 apps. The iterative extraction was done using Selenium. We used the keywords as the search keyword in the URL and connected them to the Selenium HTTP request. Once we got the entire URL of the Apps, we extracted the Metadata. We focused on the following Metadata for our research questions during data scraping. Google Play URL, App Name, Providers, Tags, Ads status, Description, Rating score, Rating Count, Installs, Size, Date of update, Content rating permission, Cost also most importantly we extracted all reviews of the apps using play-store-scraper API which has its metadata list which will be discussed in the coming section.	
\subsection{Sports app classification} We did manual labelling with the help of 2 researchers with experience in the software engineering field. As mentioned previously, we have a total of 3072 apps. Given the challenges we have in labelling the entire dataset manually for our categories' analysis is done for a sample data set. We created the sample set with 95\% confidence and 5\% interval, which gave us a piece set of 344 apps. Two members will evaluate 70\% of the sample data and derive a common understanding for labelling, and for the 30\%, all three researchers parallelly labelled. We also assessed Inter-rater reliability for the 30\% data using Cohen's Kappa method. The classification is to find the following three metrics on the sports apps:(1) Type of sports (2) Main functionality (3)Statistical/Predictive algorithm used.

\subsection{Analysis of App's  Metadata}
This section focused on the detailed analysis of the metadata of sports apps we extracted using selenium. We tried to understand the following details to leverage the market and trends of the current sports apps and their usages.

\nd a) Understanding average rating, number of installs and number of reviews associated with apps

\nd b) Distribution of paid and free apps to relate the return on investment (ROI) for the users

\nd c) The user group analysis by looking into content rating permissions
\subsection{Topic modelling on user reviews}
1) \textbf{Reviews extraction}: As a continuation of what we mentioned in the data collection part, we extracted the reviews for the sample set of 344 apps for addressing our RQ2 and RQ3. We used Google Play scraper API to extract the reviews and which returned the following metadata: 'at', 'content', 'replied', 'reply content', 'reviewCreatedVersion', 'reviewId', 'score', 'thumbsUpCount'. We tried to use most of the information to find the correlation between data and support our intuitions.

2) \textbf{Data preprocessing}: Reviews direct user feedback to developers or providers. It is the most crucial information and can be the most chaotic. Thus a detailed preprocessing of data is necessary before applying any algorithms. But the possibility of having noise in reviews is more likely, as the users use mobile phones to provide the review, which is prone to have typos [6]. The primary preprocessing removed special characters and emoticons and accepted only the English language. There were a lot of comments in local languages. For typos, we used spell checker hunspell ( the most popular open-source spell checker)[11] and replaced it with the actual or possible word. For applying topic modelling, we used further preprocessing for the NLP process, such as stop words removal using MALLET's stop words list and stemmed the words to the root words using port stemmer.

3) \textbf{Topic modelling using MALLET}: Topic modelling is a statistical method to group similar documents that discuss the same topic. MALLET is one of the successful implementations of the algorithm. Here the topic means a group of words statistically distributed in a meaningful way. To improve the topic modelling algorithm, we considered unigram, bigram, and trigram of words distribution. In topic modelling, one of the challenges is to select the number of topics for the algorithm. One of the most recognized approaches is the brute force by applying a set of values, checking the coherence score to evaluate the semantic similarity of the highly weighted words in the topics and perplexity value for the model, and selecting the K value with the best coherence score. We started the K=2 with a step size of 6 up to a stopping condition of 40. The different coherence values for different values for K. As we can see, after the K value 20, the graph reaches the convergence value for coherence and become parallel to the x-axis, so the optimal value for K is 20 with a coherence value.

Now we have the expected 20 topics that has been discussed in the reviews of the sports apps. As we mentioned previously, the topics are a group of keywords. For inferring what the topics intended by the keywords are, we need a manual evaluation. Each topic retrieves the top 10 keywords with their weights related to contributing to the topic. The labelling of the topic was done by a group of two people with expertise in app development and Google Play store platform usage. The final topics were concluded after discussion. Our conclusion was of 13 topics. We merged a few topics based on similarity and what development departments/ developers intended.

4) \textbf{Demystifying topics}:
\newline
a) Visualising the topic keywords: Visualisation enhances the understandability of the keywords to the topics. pyLDAViz package gave an interactive graph to interpret the topics to keywords.  Each bubble is a topic; if the bubble is prominent, it is one of the most important topics, and topics are expected to be distributed over all the axes rather than clustered in one.

b) Dominant topics in each review: Now, we analyze a few reviews to understand the dominant topics being discussed in the reviews. It is calculated by the percentage of contribution of each topic to that review.

c) Representative review for each topic: The keywords and their weights returned by topic modelling algorithms might not be enough to understand what the topic is all about. The most representative reviews will help us to validate and infer the topic is all about

d) Distribution of Topic across reviews: This part will help us to understand the relationship between the topic selected and the reviews represented by them. And importantly, how widely the topics are being discussed by the reviews are also being evaluated.

\subsection{Finding the reason the users are complaining most about the sports apps. }
Finding the reason the users are complaining most about the sports apps.
Although we analyzed the topics discussed in the reviews in our RQ2, this section examines the next level of the details to understand why users hate sports apps. Each review is associated with rating, and rating is considered the quantifiable measure of how the users feel, and reviews are the descriptive way of the same. Hypothetically, both are significantly correlated. The reviews with low ratings should be bad reviews, and those with high ratings should be good. However, the cases are different. There is a lot of noise in Text- Rating- Consistency( TRC), as explained in the paper [Cite]. The approach we used to mitigate this challenge is to evaluate the sentiment of the reviews and correlate it with the review ratings available.
\subsubsection{The sentiment of the reviews and the user ratings}: Understanding and making the sentiment of users' emotions while writing the reviews can aid in understanding what they are conveying through the reviews. 

\newline
a) \textbf{Preprocessing}: User reviews are one of the pure forms of natural language; it contains a lot of noises ( Which we mentioned in the topic modelling section ), and the tricky part of natural language - the irony. We used the NLTK sentimental analysis library to return the positive, negative, and compound values of each review. To get rid of the outlier, we focused on the positive values and the rating associated with the review. If the rating is less than or equal to 2 and the positive sentiment of the review is not less than 50, we consider it as outliers.

\newline
b) \textbf{Sentiment analysis}: We analyzed the sentiment of the reviews and plotted against the user reviews to understand the users' emotions while writing the review.

\subsubsection{The factors to hate}

\newline
a) \textbf{Data collection}: We have the bad reviews without the outliers and the topics associated with each review from our previous sections. Also, we considered these given research papers to understand the common hate factors among the available apps and another category of apps to list out the significant points to the differences in the disturbing characteristics for the users.
b) \textbf{Analysis}: We compared the topics that are mainly being discussed in the low rated reviews. To understand more on reviews of complaints we did Qualitative analysis why these topics are associated with negative sentiment and low ratings: use a stratified sampling of the curated data set  with 95\% confidence level and 5\% confidence interval.
